RAP-WAM: Learning World-Action Models through Predictive Rehearsal and Action Perturbations

World-action models learn to predict future images and robot actions together, yet lower image error need not yield more accurate actions. Training must both prepare the model for imperfect predicted conditions and emphasize visual predictions that change with the action; reconstruction loss alone does not supply both signals. We introduce RAP-WAM, which combines predictive rehearsal and matched action perturbations to guide world-action model training. Rehearsal trains continuations conditioned on generated observations and accumulates recurring errors into a spatial prior, while matched action perturbations hold the scene and noise fixed to identify action-sensitive visual predictions. Combined with current prediction error, these signals guide spatial visual and temporal action supervision without region annotations or a separate scoring network. Initialized from Awomo-0.5, RAP-WAM raises average success on RoboDojo from 22.80% to 27.55%. Real-robot evaluation of the complete system yields 89.00% task-macro-average success across 15 tasks. Videos and further details are available on the project website: https://rapwam.github.io/.

==> float_page_targets.tex <==
% Earliest physical page per float. Preserve natural text flow without blank-page padding.
% Labels attach targets to float boxes; parbox labels use the amsmath ltx alias.
\makeatletter
\expandafter\def\csname paper@target@fig:overview\endcsname{3}
\expandafter\def\csname paper@target@tab:primary-leaderboard\endcsname{6}
\expandafter\def\csname paper@target@fig:allocation-fingerprint\endcsname{7}
\expandafter\def\csname paper@target@fig:light-credit-dynamics\endcsname{8}
\expandafter\def\csname paper@target@fig:real-robot-15x6\endcsname{9}

\let\paper@label\label
\def\label#1{%
 \ifcsname paper@target@#1\endcsname
  \expandafter\xdef\csname paper@box@\number\@currbox\endcsname{\csname paper@target@#1\endcsname}%
 \fi
 \paper@label{#1}}
\let\paper@xfloat\@xfloat
\def\@xfloat#1[#2]{\paper@xfloat{#1}[#2]%
 \expandafter\gdef\csname paper@box@\number\@currbox\endcsname{0}}
\def\paper@ifearly#1{%
 \ifcsname paper@box@\number#1\endcsname
  \ifnum\c@page<\csname paper@box@\number#1\endcsname\relax
   \expandafter\expandafter\expandafter\@firstoftwo
  \else\expandafter\expandafter\expandafter\@secondoftwo\fi
 \else\expandafter\@secondoftwo\fi}
\let\paper@addtocurcol\@addtocurcol
\def\@addtocurcol{\paper@ifearly\@currbox
 {\@insertfalse\@resethfps\@cons\@deferlist\@currbox}
 {\paper@addtocurcol}}
\let\paper@addtonextcol\@addtonextcol
\def\@addtonextcol{\paper@ifearly\@currbox
 {\@cons\@deferlist\@currbox}
 {\paper@addtonextcol}}
\let\paper@testfp\@testfp
\def\@testfp#1{\paper@testfp#1\paper@ifearly#1{\@testtrue}{}}
% A forced flush must make progress even on the first pass, when missing
% bibliography/cross-references can shorten the document below target pages.
\let\paper@makefcolumn\@makefcolumn
\def\@makefcolumn#1{%
 \begingroup
  \@fpmin -\maxdimen
  \def\@testfp##1{\paper@ifearly##1{\@testtrue}{}}%
  \@tryfcolumn#1%
 \endgroup
 \if@fcolmade\else
  \global\let\paper@hasearly\@secondoftwo
  \begingroup
   \def\@elt##1{\paper@ifearly##1{\global\let\paper@hasearly\@firstoftwo}{}}%
   #1%
  \endgroup
  \paper@hasearly
   {\global\setbox\@outputbox\vbox to\@colht{\vfil}\global\@fcolmadetrue}%
   {\paper@makefcolumn#1}%
 \fi}
\let\ltx@label\label
\makeatother

\newcommand{\paperstartpage}[1]{\par\ifnum\value{page}<#1\relax\clearpage\loop\ifnum\value{page}<#1\relax\null\newpage\repeat\fi}

